Stratosphere: Finding Vulnerable Cloud Storage Buckets

Misconfigured cloud storage buckets have leaked hundreds of millions of medical, voter, and customer records. These breaches are due to a combination of easily-guessable bucket names and error-prone security configurations, which, together, allow attackers to easily guess and access sensitive data. In this work, we investigate the security of buckets, finding that prior studies have largely underestimated cloud insecurity by focusing on simple, easy-to-guess names. By leveraging prior work in the password analysis space, we introduce Stratosphere, a system that learns how buckets are named in practice in order to efficiently guess the names of vulnerable buckets. Using Stratosphere, we find wide-spread exploitation of buckets and vulnerable configurations continuing to increase over the years. We conclude with recommendations for operators, researchers, and cloud providers.

==> acknowledgements.tex <==
\textbf{Acknowledgements}\quad 


==> scraps.tex <==

{\centering
\begin{table}[h!]
    \centering
    \begin{tabular}{l l l l }
    \toprule
        Characters & \% Existing & \% Public \\
        \midrule
         4 & 2.69\% & 0.607 \% \\
         5 & 0.139\% & 0.0185\%  \\
         6 & 0.00407 \% & 0.00037 \% \\
         7 & 0.000741 \% & None found \\
         8 & None found &  None found  \\
         9 & None found  & None found \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Random Scanning}---The hit-rate of generating random alpha-numeric bucket-name sequences decays exponentially as the bucket length increases. We show the proportion of buckets found with 1,000,000 Random Guesses per length, across AWS,GCP, and Alibaba. \todo{remove? dont talk about random that much anymore} }
    \label{tab:random}
\end{table}
}

{\centering
\begin{table*}[h!]
    \centering
    \begin{tabular}{lll |llll }
    \hline
          Name & \% Easy & AVG& Name &\% Hard & AVG   \\
          Structure & Names & $\log_{10}(Guess)$  & Structure & Names & $\log_{10}(Guess)$ \\
        \hline
         (rand) &   12.9\% & 4.7 & (rand) &  21.5\% & 18.2\\
         \hline
          Length 4 & 51\%&4 &  Length 18 & 37.4\% & 18 & \\
          Length 5 & 16.9\%&5 &  Length 25 & 19.2\% & 25 & \\
          Length 3& 10.1\%&3 &  Length 14 & 7.5\% & 14&  \\
          %Length 6& 9.2\% &6 & Length 20 & 7.2\% & 20& \\
          %Length 7 & 6\%& 7&  Length 10 & 6.3\% & 10& \\
         \hline
         (rand,corpus) &    10\% &6.7 & (rand,corpus,rand) &     8.1\%&18.0\\
         \hline
          (rand,``test'') & 6.8\% & 6.4 &  (rand,``asset'',rand) & 1.9\% & 12.0& \\
          (rand,``dev'') & 3.2\% & 6.4 & (rand,``upload'',rand) & 1.8\%&12.1 & \\
          (rand,``bucket'') & 3.1\% & 7.6& (rand,``log'',rand) & 1.1\%&18.5 & \\
          %(rand,``backup'') & 2.7\% & 6.3& (rand,``prod'',rand) & 0.9\% & 15& \\
          %(rand,``data'') & 2.6\% &  6.2& (rand,``bucket'',rand)&  0.8\%& 13& \\
         \hline
         (corpus,rand) &   5.2\% &6.4 & (corpus,rand) &  3.9\%&12.9\\
         \hline
          (``test'',rand) & 5.5\% & 6.0 &  (``test'', rand) & 2.0\% & 11.4 & \\
          (``bucket',rand)& 1.7\% & 7.2 &  (``static'',rand) & 1.8\% & 12.3 & \\
          (``backup',rand) & 1.6\% & 6.1& (``img'',rand) & 1.1\% & 13.5& \\
          %(``dev'',rand) & 1.6\% &6.1 &  (``media'',rand) & 1.1\% & 13.6& \\
        \hline
        (corpus,corpus,corpus) &    4.2\% & 8.5 & (corpus,rand,corpus) &  3.6\%&12.4\\  
        \hline
         (dict,``-'',dict) & 31.1\% & 8.5& (``staging'',rand,``appspot.com'')& 0.6\% & 23.1 \\
         (dict,``-'',tech-term) & 11.2\% & 8.1&  (tech terms, ``s.'',top domains) & 0.5\% & 10.3 \\
         (password,``-'',dict) & 9.5\% & 8.5&  (``test'',rand,``bucket'') & 0.3\% &11.9 \\
        \hline
        (corpus,corpus) &   2.4\% & 5.8 & (rand,corpus,corpus,corpus) &   3.1\%& 14.3\\  
        \hline
         (dict,``2'') & 1.6\% &  4.7 &  (rand,``terraform'',``-'',``state'') & 1.1\% & 15.0 & \\  
         (dict,``test'') & 1.6\% & 5.2 &  (rand,``test'',``-'',``bucket'') & 0.9\% & 13.4 & \\ 
         (dict,``bucket'') & 1.4\% & 6.7 &  (rand,``static'',``-'',``assets'') & 0.8\% & 13.0 & \\ 
    \end{tabular}
    \caption{\textbf{Bucket Naming Schemes}---\todo{change to just include schemes for all names found in passive sources?}The most common naming scheme of buckets for both easily guessable (< $10^{10}$) and difficultly guessable (>= $10^{10}$) is a concatenation of random ( denoted by``rand'') alpha-numeric-symbol strings and words found in a corpus.  Harder to guess bucket names are longer in length and contain more tokens. }
    \label{tab:naming_schemes}
\end{table*}
}


{\centering
\begin{table}[h!]
    \centering
    \begin{tabular}{lll }
    \hline
          Name &\% Hard & AVG    \\
           Structure & Names &  $\log_{10}(Guess)$ \\
        \hline
         (rand) &  43.3\% & 19.0\\
         \hline
          Length 18 & 42.6\% & 18.0 \\
          Length 25 & 22.2\% & 25.0  \\
          Length 20 & 8.3\% & 20.0 \\
         \hline
         (rand,corpus,rand) &     18.0\%&19.44\\
         \hline
         (rand,``eca'',rand) & 0.8\% & 20.0 \\
         (rand,``ace'',rand) & 0.7\%&19.8  \\
         (rand,``eno'',rand) & 0.6\%&17.4  \\
         \hline
        (rand,corpus) &   3.5\%&15.6\\  
        \hline
        %(rand,``test'') &  5.0\%& 10.8 \\
        %(rand,``bucket'') &  2.7\%& 11.4 \\
        %(rand,``prod'') &  2.0\%& 10.9 \\
        %(rand,``images'') & 1.7\%& 11.2 \\
        %(rand,``dev'') &  1.6\%& 10.5 \\
        (corpus,rand) & 3.4\%& 15.8\\  
        \hline
         (``test'',rand) & 0.9\%& 10.8\\  
         (``xiao'',rand) & 0.6\%& 12.4\\  
         (``hong'',rand) & 0.6\%& 11.4\\  
        \hline
        (corpus,rand,corpus) & 2.7\%&11.6\\
        \hline
        (dict,``-bucket-'',tech term) & 1.1\% & 13.5  \\
         (dict,``-data-'',tech term) & 0.9\% & 11.4 \\
         (``bucket'',rand,``test'') & 0.8\% & 13.3 \\
         \hline
        (corpus,corpus,rand) & 1.4\%&13.8\\
        \hline
        (rand,corpus,corpus) & 1.3\%&14.0\\
        \hline
        (corpus,corpus,corpus) & 1.1\%&10.8\\
        \hline
         (rand,corpus,corpus,rand) & 0.9\%&19.2\\
        \hline
         (rand,corpus,corpus,corpus) & 0.8\%&13.2\\
        \hline
         (rand,``test'',``-''``bucket'') & 3.0\% & 12.4  \\
         (rand,``bucket'',``-'', ``test'') & 2.5\% & 12.4  \\
         (rand,``static'',``-'', ``assets'') & 2.0\% & 12.4  \\
        \hline


    \end{tabular}
    \caption{\textbf{Token PCFG Bucket Naming Schemes}---The Token PCFG finds difficultly-guessable bucket names that are similar in structure to the names found in passive DNS sources (Table~\ref{tab:naming_schemes}).}
    \label{tab:naming_schemes_pcfg}
\end{table}
}

%\begin{figure}[h]
%    \centering
%    \includegraphics[ width=3in]{figures/scanning_campaign.pdf}
%    \caption{\textbf{Bucket Warning Over Time}---message uploads are often clustered around specific dates, with the top day most warned (September 28,2020) making up 24\% of all warning messages dropped across the last 10 years. }
%    \label{fig:scanning_camp}
%\end{figure}


In total, we analyze 20~different permission requests, representing all request methods that return permission metadata about a serverless storage bucket. We request these methods against all public buckets, as well as a sample of 100,000 private buckets.
Of the 20~permissions, 1~ are enabled on at least one bucket. The most common permissions, "get\_bucket\_tagging" (i.e., return optional bucket tags) and "get\_bucket\_acl" (i.e., return the bucket access control list), are enabled on 11\% and 10.6\% of public buckets respectively.
\todo{mention info leak in tagging where clients were revealed from buckets. }

Of all public AWS S3 buckets, 24\% allow the the bucket ACL to be read. \todo{why is this so much larger than the 10.6 above? can we have the stat for google?}. We identify the most vulnerable permissions to be WRITE (i.e., allowing any upload or deletion of files to a bucket), WRITE\_ACP (i.e., allowing any permission to be turned on or off, including WRITE), and FULL\_CONTROL (i.e., allowing any permission in general, including WRITE\_ACP and WRITE). We also identify the most vulnerable User Groups to be ``AllUsers'' (i.e., allowing anyone with the bucket name to be bound by a permission) and the---confusingly---labeled ``Authenticated'' (i.e., allowing anyone with a registered cloud account to be bound by a permission). 
We note that, for all intents and purposes, giving permissions to an ``Authenticated'' user group allows no extra security as anyone in the public can always create an anonymous cloud account. 



\begin{table*}
\centering


\caption{State of common cloud storage providers}\label{title}
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
Product               & Public access & Public default & Bucket listing & Global namespace & Account ID & Random ID & Example bucket                                                                        &                                                                      \\ \hline
%\endfirsthead
%
%\endhead
%
Amazon S3             & Yes                  & No                & Yes                   & Yes              & No                 & No                & bucket.s3.amazonaws.com                                                               &                                                                      \\ \hline
Google Cloud Storage  & Yes                  & No                & Yes                   & Yes              & No                 & No                & bucket.storage.googleapis.com                                                         &                                                                      \\ \hline
Digital Ocean Spaces  & Yes                  & No                & Yes                   & No               & No                 & No                & bucket.nyc3.digitaloceanspaces.com                                                    &                                                                      \\ \hline
Azure Blob Storage    & Yes                  & No                & Yes                   & No               & Yes (container)    & No                & bucket.blob.core.windows.net/container %\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} bucket.blob.core.windows.net/container} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }} 
\\ \hline
Alibaba OSS           & Yes                  & No                & No                    & Yes              & No                 & No                & bucket.oss-us-west-1.aliyuncs.com                                                     &                                                                      \\ \hline
Oracle Object Storage & Yes                  & No                & Yes                   & No               & Yes                & No                & objectstorage.us-ashburn-1.oraclecloud.com/n/idigcj0ngbao/b/bucket/o/                 &                                                                      \\ \hline
\end{tabular}
\end{adjustbox}
\end{table*}



\begin{figure}[h]
\includegraphics[scale=0.3]{figures/file-types.png}
\caption{Most common exposed file types (as of 12/09/2020)}
\end{figure}
\label{fig:file_extensions}


\textbf{Limitations}\quad Our work was limited in several aspects for which we intend to improve in future work. Due to subtleties in S3's APIs and permissions, there may have been cases where we failed to identify buckets that did exist, or labeled buckets that had some level of public access as private. First, while we made every request with the validator to the region-agnostic domain ``s3.amazonaws.com'', there exist cases where the bucket can only be accessed by making a request specifically to the bucket's region.\li{in the methodology section where we describe the exact experiment we did (e.g., the exact days we scanned etc) we should remember to mention the region we scanned from} In particular, regions that have been created after March 20, 2019, which at the time of writing are only \textit{me-south-1} and \textit{ap-east-1}, require making requests directly to the region-specific host \cite{s3Naming}. 
In future work, we intend to attempt making HEAD requests to several common files in order to determine if any files can be accessed. \li{what did previous work do? do we want to do this for the paper? Jack: Continella did not attempt to read files from buckets that did not have directly listings. They did make HEAD requests in order to check if files from buckets with directory listings were accessible, which we could do at scale}

\label{sub:sub:sec:category_buckets}
Of the 2.1M~buckets exposed in our study, 173K (13\%) have publicly listable files (Table~\ref{table:data_breakdown} and Table~\ref{table:gen_buckets}).
Some buckets may intentionally allow public read access, such as buckets used to host public websites or to share public data sets; however, we find hosted file extensions that should never be public. To better understand whether accessible buckets pose a security risk, we investigate the types of files exposed in public buckets by collecting file metadata for up to 100K files in public bucket. In total, we collect metadata for 1.1B~files from 135K~buckets.


\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/bucket_categories.pdf}
    \caption{\textbf{Categories of public buckets per source}---The fraction of categorizable buckets (across all time) varies widely across sources, between 80\% (Continella) to 35\% (Token PCFG).}
    \label{fig:bucket_categories}
\end{figure}

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=\linewidth]{figures/cats_overtime.pdf}
%    \caption{\textbf{Categorization of buckets over time}---In the past decade, the popularity of hosting webpages has increased over 5x. }
%    \label{fig:bucket_categories_overtime}
%\end{figure}

We are able to categorize 58\% of all public buckets as belonging to a specific use case: of these, 50\% primarily store images, 18\% host web-page material, and 16\% store documents (Figure~\ref{fig:bucket_categories}). The remaining 42\% of buckets contain a mix of files, but most commonly host images, followed by documents and video files. These remaining buckets generally contain files across several categories with the most popular containing images and video files, or images and documents. 




% The "users.txt" category encompasses 1,956 S3 buckets, all of which are named for large corporations and contain a single text file, "users.txt". It is likely that the same individual operates these buckets --- all "users.txt" files were created within a 2-week timespan in December 2019, have the same file size, and have the same file hash. Further, no buckets allow reading their ACL, which would be highly unlikely for a random distribution of buckets. Given these factors, we suspect that these buckets are used as honeypots to collect information about S3 traffic.

%The distribution of categories varies widely based on the bucket source. Continella, for example, generates the least diverse buckets, with over 60\% of buckets belonging to the "images" category and nearly 80\% of buckets being categorizable. Conversely, farsight buckets are the least categorizable, with fewer than 50\% of buckets belonging to a category. Sources that rely on web scraping, such as Bing, contain a higher percentage of web-related buckets (webpage and wordpress categories). This suggests that GrayHat, which has the highest percentage of webpage buckets, may also rely on web scraping for a portion of its bucket discovery.


Across cloud providers, we see variation in types of categories present: 6\% of AWS buckets belong to the "documents" category, compared to 16\% of GCP buckets. AWS appears more widely used for web pages among public buckets, with 14\% compared to GCP's 6\%. Alibaba is the least categorizable, with nearly 60\% of buckets being unidentifiable, compared 44\% for AWS and 40\% for GCP. We suspect that some of this difference may be due to a majority of buckets on Alibaba being non-English language, while some of our tags rely on English keywords. When categorizing buckets by creation date, over the past decade, the popularity of hosting web pages has increased over 5~times, while storing Wordpress content has nearly disappeared since 2016. Storing logs and documents publicly has also decreased in popularity over the years. In 2020, 95\% of categorized buckets store webpages or images. 


\section{Security of Serverless Storage}


%Across the 10 buckets, 80\% are categorized as documents and contain PDFs of the sensitive data. 


%We find no notable differences in bucket naming patterns (Section~\ref{sub:sec:naming_patterns}) across categories of buckets.

%\subsection{Temporal Analysis of Bucket Modification}
%We extract the bucket creation date and last updated timestamp in the provided file metadata of all public buckets. 
%Across all public buckets found, we discover 42\% are never modified after the day they are created and 60\% are modified less than three times. 
%We plot the creation of all stale buckets (i.e., buckets never updated after their creation day) in Figure~\ref{fig:bucket_misconfigs_time} and discover that on average, 27\% of public buckets created every month in the past 15~years are never touched after the day they were created. Moreover, 20\% of buckets created 10~years ago have never been touched since.
%When breaking down bucket activity by bucket category, we find 64\% of buckets hosting primarily keys, 63\% webpages, and 46\% images are never modified the day after the bucket is created. However, only 1.7\% of buckets hosting primarily logs are never modified.

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=\linewidth]{figures/created-v-neverupdated.pdf}
%    \caption{\textbf{Bucket Staleness}---On average, 27\% of public buckets created every month are never touched after the day they were created. Moreover, 20\% of buckets created 10~years ago have never been touched since.}
%    \label{fig:bucket_misconfigs_time}
%\end{figure}

%\subsection{Vulnerable Permissions Analysis}
%\label{sub:sec:perm_analysis}


 

%We assess that certain permissions are more rare to misconfigure than others, and hence those misconfigurations tend to stem from one specific organization's missteps. For instance, of 308 buckets across all platforms that have the "GetBucketTagging" operation enabled, 84 (27\%) belong to a single company that provisions buckets for its clients, with each tag containing a client name. The same pattern is present for the GetBucketLifecycleConfiguration, with 84 of 366 misconfigured buckets belonging to the same company. There is a much longer tail of organizations for buckets with open access control lists. Restricting to S3 (as only S3 exposes the owner's account ID), we observe that 60\% of buckets with misconfigured access control lists belong to a unique organization, with the remaining 40\% of buckets created by 20\% of organizations. Thus, the issue of misconfigured bucket access control lists appears to be a widespread problem across organizations on S3.




%\subsubsection{ETag Side-channel}
%\label{sub:sub:etag}

%When listing all objects in a bucket (i.e., fetching file metadata), AWS and GCP provide an ``ETag''---a unique and deterministic file identifier that is often simply the MD5 digest of file contents~\cite{s3ETag, kaminsky2005md5}. %and is used by clients for verification in sync operations. However, previous work has showed that using such ETags is insecure, as content within a file can be deciphered by reversing the MD5 hash~\cite{kaminsky2005md5}---even with an S3 Encryption Client~\cite{s3Encrypt}---and reverse looking-up the MD5 hash using cached repositories~\cite{rainbow}. 
%We discover a new side-channel to decipher the contents of a private file with an available ETag: using ETag collisions across other public buckets.
%By searching (e.g., across other buckets, Google) for an ETag associated with a private file, we can discover other public buckets that allow an attacker to read the contents of a file with the same ETag. Among all our data sources, 
%9\% of ETags are found in more than one bucket and 48\% of publicly-listable buckets contain an ETag found in another public bucket.

%Across all GCP buckets that allow for objects to be listed (i.e., public) but do not allow for objects to be read, we discover 22.5\%  contain at least one ETag that is found in another public bucket with object read permissions, and is thus vulnerable to the ETag side-channel. Furthermore, we hypothesize that the fraction of vulnerable buckets is actually much higher, as particular ETags can be web searched and thus increase the likelihood of finding a public bucket with the particular ETag. Due to this information leakage, we implore AWS and GCP to consider not returning ETags for files that the requester cannot access.




